Measurement of the Cosmic Ray and Neutrino-Induced Muon Flux at the Sudbury Neutrino Observatory

Results are reported on the measurement of the atmospheric neutrino-induced muon flux at a depth of 2 kilometers below the Earth's surface from 1229 days of operation of the Sudbury Neutrino Observatory (SNO). By measuring the flux of through-going muons as a function of zenith angle, the SNO experiment can distinguish between the oscillated and un-oscillated portion of the neutrino flux. A total of 514 muon-like events are measured between $-1 \le \cos{\theta}_{\rm zenith} \le 0.4$ in a total exposure of 2.30\times 10^{14}$ cm$^{2}$ s. The measured flux normalization is $1.22 \pm 0.09$ times the Bartol three-dimensional flux prediction. This is the first measurement of the neutrino-induced flux where neutrino oscillations are minimized. The zenith distribution is consistent with previously measured atmospheric neutrino oscillation parameters. The cosmic ray muon flux at SNO with zenith angle $\cos{\theta}_{\rm zenith} > 0.4$ is measured to be $(3.31 \pm 0.01 {\rm (stat.)} \pm 0.09 {\rm (sys.)}) \times 10^{-10}~\mu$/s/cm$^{2}$.

==> table_atmo_results.tex <==
%
%  Atmospheric results table
%  For the 3-Phase
%
\begin{table}[htdp]
\caption{Summary of fit results for SNO only data and with the oscillations parameters constrained to the global best fit oscillation parameters of Super-Kamiodande and MINOS (see text for details).  The no oscillations fit assumes only a change in scaling for the number of events predicted.  All measured fluxes are compared to Bartol flux calculations.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline \hline
Fit Type & $\Phi_0$ & $\Delta m^2$ & $\sin^2{2\theta}$ & $\Delta{\cal L}$ \\
\hline
SNO Only & \normalization & \msqatm & \thetaatm & -- \\
With SK and MINOS constraints & \normalizationconst & Constrained & Constrained & - \\
\hline
No Oscillations & & N/A & N/A & 9.9 \\
\hline \hline
\end{tabular}
\end{center}
\label{tab:fluxes}
\end{table}%

